MUSE Analysis of Gas around Galaxies (MAGG) -- I: Survey design and the environment of a near pristine gas cloud at z~3.5

We present the design, methods, and first results of the MUSE Analysis of Gas around Galaxies (MAGG) survey, a large programme on the Multi Unit Spectroscopic Explorer (MUSE) instrument at the Very Large Telescope (VLT) which targets 28 z > 3.2 quasars to investigate the connection between optically-thick gas and galaxies at z~3-4. MAGG maps the environment of 52 strong absorption line systems at z > 3, providing the first statistical sample of galaxies associated with gas-rich structures in the early Universe. In this paper, we study the galaxy population around a very metal poor gas cloud at z~3.5 towards the quasar J124957.23-015928.8. We detect three Lyman alpha emitters within <200km/s of the cloud redshift, at projected separations <185 kpc (physical). The presence of star-forming galaxies near a very metal-poor cloud indicates that metal enrichment is still spatially inhomogeneous at this redshift. Based on its very low metallicity and the presence of nearby galaxies, we propose that the most likely scenario for this LLS is that it lies within a filament which may be accreting onto a nearby galaxy. Taken together with the small number of other LLSs studied with MUSE, the observations to date show a range of different environments near strong absorption systems. The full MAGG survey will significantly expand this sample and enable a statistical analysis of the link between gas and galaxies to pin down the origin of these diverse environments at z~3-4.

==> tablespectra.tex <==
\begin{table*}
\centering
\caption{Summary of the archival quasar spectroscopy used in this survey.
  The table lists: the quasar name; the instrument name; the spectral resolution (range is used if dependent on instrument arm);
  the wavelength range covered by the spectrum (gaps may be present); the typical $S/N$ per pixel representative of the Ly$\alpha$ forest, away from saturated absorption lines (actual wavelengths given in parenthesis, in \AA);
the typical $S/N$ per pixel measured representative of the continuum redward to the quasar Ly$\alpha$ (actual wavelengths given in parenthesis, in \AA) the pixel velocity dispersion (range is used if arm dependent).}\label{tab:qsospectra}
\begin{tabular}{llccrrr} 
\hline
Name & Instrument & Resolution          & Wavelength Range & $S/N_{\rm blue}$  & $S/N_{\rm red}$ & Dispersion      \\
     &            &                     &       (\AA)      &               &              &    ($\rm km~s^{-1}$) \\

\hline
\hline
J010619.24+004823.3      &  MIKE & 28,000;22,000 & 3450$-$8100 &  7 (6280)  & 10 (7000)  &    4.2 \\
                         &  ESI  & 5,400           & 3927$-$11068&  31 (6280) & 36 (7000)  &    10  \\
\hline
J012403.77+004432.7      &  UVES & 40,000 & 4173$-$6813 & 27 (5500) & 23 (6500)  &    2.5  \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$24800 & 31 (5500) & 33 (6500)  & 20;11;19   \\	 
\hline
J013340.31+040059.7      &  UVES & 40,000 & 4665$-$10425& 20 (5500) & 15 (7000)  &    2.5  \\	 
                         &  HIRES& 49,000 & 4160$-$8720 & 14 (5500) & 15 (7000)  &    1.3  \\	 
                         &  ESI  & 5,400 & 3927$-$11068& 25 (5500) & 30 (7000)  &  10  \\
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 55 (5500) & 54 (7000)  & 20;11;19   \\	 
\hline
J013724.36$-$422417.3    &  UVES & 40,000 & 4265$-$9765 & 11 (5700) & 14 (6500)  &    2.5 \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 12 (5700) & 22 (6500)  & 20;11;19   \\	 
\hline
J015741.56$-$010629.6    &  HIRES& 37,000 & 3890$-$6290 & 12 (5000) & 18 (5850)  &	2.6 \\
                         &  ESI  & 5,400 & 3927$-$11068& 12 (5000) & 17 (5850)  &  10  \\
                         &  X-SHOOTER & 4350;7450;8100 & 3150$-$24800 & 48 (5000) & 45 (5850)  & 18;11;11   \\	 
\hline
J020944.61+051713.6      &  UVES & 40,000 & 4577$-$6809 & 19 (5450) & 21 (6500)  &	2.5  \\	 
                         &  HIRES& 49,000 & 5190$-$6300 & 35 (5450) & 65 (6500)  &	1.3  \\	 
                         &  ESI  & 8,000 & 3927$-$11068& 21  (5450) & 29 (6500)  &  10  \\
                         &  X-SHOOTER & 6700;11400;8100 & 3150$-$24800 & 37 (5450) & 57 (6500)  & 18;11;11   \\	 
\hline
J024401.84$-$013403.7    &  UVES & 40,000 & 4533$-$6811 & 15 (5550) & 10 (6500)  &	2.5  \\	 
                         &  HIRES& 49,000 & 4470$-$7050 & 15 (5550) & 20 (6500)  &	2.6  \\	 
                         &  ESI  & 8,000 & 3927$-$11068& 29 (5550) & 35 (6500)  & 10  \\
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 35 (5550) & 33 (6500)  & 20;11;19   \\	 
\hline
J033413.42$-$161205.4    &  UVES & 40,000 & 4700$-$10425& 18 (6000) & 21 (6900)  &	2.5  \\	 
                         &  ESI  & 5,400 & 3927$-$11068& 35 (6000) & 58 (6900)  &  10  \\
\hline
J033900.98$-$013317.7    &  UVES & 44,400 & 3759$-$10255& 16 (4650) & 27 (7000)  &	2.5 \\	 
                         &  HIRES& 37,000 & 3734$-$7200 & 20 (4650) & 32 (6050)  &	2.6  \\	 
\hline
J094932.26+033531.7      &  MIKE & 40,000;30,000& 3300$-$7420 & 13 (5700) & 19 (6800)  &    4.2  \\
\hline
J095852.19+120245.0      &  HIRES& 37,000 & 3625$-$8560 & 38 (5000) & 53 (5950)  &	2.6	 \\
\hline
J102009.99+104002.7      &  HIRES& 37,000 & 3650$-$6790 & 36 (4500) & 50 (5500)  &    2.6 \\
\hline
J111008.61+024458.0      &  MIKE & 40,000;30,000 & 3300$-$7420 &  9 (5800) & 11 (6800)  &    4.2  \\
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 23 (5800) & 35 (6800)  & 20;11;19   \\	 
\hline
J111113.79$-$080402.0    &  UVES & 40,000 & 4395$-$10425& 22 (5500) & 32 (7000)  &	2.5  \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$24800 & 45 (5500) & 45 (7000)  & 20;11;19   \\	 
\hline
J120917.93+113830.3      &  UVES & 40,000 & 3510$-$7006 &  6 (4400) & 11 (5500)  &	2.5  \\	 
                         &  HIRES& 37,000 & 3530$-$6410 & 30 (4400) & 36 (5500)  &	2.6  \\	 
\hline
J123055.57$-$113909.3    &  UVES & 40,000 & 3886$-$6810 & 12 (5000) & 14 (6000)  &	2.5  \\	 
\hline
J124957.23$-$015928.8    &  UVES & 40,000 & 3729$-$6811 & 47 (5000) & 46 (6000)  &	2.5  \\	 
                         &  HIRES& 49,000 & 4110$-$8675 & 14 (5000) & 18 (6050)  &	2.6  \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$24800 & 40 (5000) & 26 (6050)  & 20;11;19   \\	 
\hline
J133254.51+005250.6      &  HIRES& 49,000 & 4118$-$8560 &  9 (5000) & 12 (6050)  &    1.3	 \\
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$24800 & 73 (5000) & 45 (6050)  & 20;11;19   \\	 
\hline
J142438.10+225600.7      &  UVES & 40,000 & 3290$-$6806 & 105 (5000) &130 (6000) &	2.5  \\	 
                         &  HIRES& 37,000 & 3570$-$7295 & 226 (5000) &345 (6050) &	2.6  \\	 
                         &  ESI  & 5,400 & 3927$-$11068& 41 (5000) & 57 (6000)  & 10  \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\contcaption{Summary of the archival quasar spectroscopy used in this survey.
  The table lists: the quasar name; the instrument name; the spectral resolution (range is used if dependent on instrument arm);
  the wavelength range covered by the spectrum (gaps may be present); the typical $S/N$ per pixel representative of the Ly$\alpha$ forest, away from saturated absorption lines (actual wavelengths given in parenthesis, in angstrom);
the typical $S/N$ per pixel measured representative of the continuum redward to the quasar Ly$\alpha$ (actual wavelengths given in parenthesis, in angstrom); the pixel velocity dispersion (range is used if arm dependent).}\label{tab:qsospectra2}
\begin{tabular}{llccrrr} 
\hline
Name & Instrument & Resolution          & Wavelength Range & $S/N_{\rm blue}$  & $S/N_{\rm red}$ & Dispersion      \\
     &            &                     &       (\AA)      &               &              &    ($\rm km/s$) \\

\hline
\hline
J162116.92$-$004250.8    &  UVES & 40,000 & 3735$-$9466 & 61 (5500)  & 96 (6000)  &	2.5  \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$24800 & 55 (5500) & 37 (6000)  & 20;11;19   \\	 
\hline
J193957.25$-$100241.5    &  UVES & 39,600 & 3821$-$6812 & 81 (5500)  & 85 (6500)  &	2.5  \\	 
                         &  HIRES& 37,000 & 3505$-$6750 & 96 (5500)  &105 (6500)  &	2.6  \\	 
\hline
J200324.14$-$325144.8    &  UVES & 40,000 & 4152$-$10425& 83 (5400)  & 78 (6500)  &	2.5  \\	 
                         &  ESI  & 8,000 & 3927$-$11068& 46 (5400) & 51 (6500)  & 10  \\
\hline
J205344.72$-$354655.2    &  MIKE & 28,000;22,000 & 3340$-$9422 &  8 (4950)  & 10 (6500)  & 4.2 \\
\hline
J221527.29$-$161133.0    &  UVES & 40,000 & 4276$-$9766 & 10 (5750)  & 18 (6600)  &	2.5  \\	 
                         &  HIRES& 49,000 & 4470$-$6920 & 11 (5750)  & 14 (6600)  &	2.6  \\	 
                         &  ESI  & 8,000 & 3927$-$11068& 15 (5750) & 21 (6400)  & 10  \\
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 20 (5750) & 37 (6400)  & 20;11;19   \\	 
\hline
J230301.45$-$093930.7    &  MIKE & 28,000;22,000 & 3320$-$8108 & 17 (5200)  & 21 (5700)  & 4.2 \\
                         &  HIRES& 37,000 & 3878$-$8351 & 71 (5200)  & 75 (6050)  & 2.6 \\
\hline
J231543.56+145606.4      &  HIRES& 37,000 & 3853$-$7817  & 18 (5100)  & 18 (6050)  &	2.6 \\
                         &  ESI  & 8,000 & 3927$-$11068& 13 (5100) & 18 (6050)  & 10  \\
\hline
J233446.40$-$090812.2    &  UVES & 40,000 & 3820$-$10425& 38 (4500) & 45 (6500)  &	2.5  \\	 
                         &  HIRES& 49,000 & 3794$-$8336& 34 (4500) & 44 (6500)  &	2.6  \\	 
\hline
J234913.75$-$371259.2    &  UVES & 40,000 & 4639$-$6409 &  7 (6000) &  -  &	2.5 \\	 
                         &  X-SHOOTER & 4350;7450;5300 & 3150$-$18000 & 16 (6000) & 25 (6700)  & 20;11;19   \\	 
\hline
\end{tabular}
\end{table*}

